A supreme test for periodic explosive GARCH

We develop a uniform test for detecting and dating explosive behavior of a strictly stationary GARCH$(r,s)$ (generalized autoregressive conditional heteroskedasticity) process. Namely, we test the null hypothesis of a globally stable GARCH process with constant parameters against an alternative where there is an 'abnormal' period with changed parameter values. During this period, the change may lead to an explosive behavior of the volatility process. It is assumed that both the magnitude and the timing of the breaks are unknown. We develop a double supreme test for the existence of a break, and then provide an algorithm to identify the period of change. Our theoretical results hold under mild moment assumptions on the innovations of the GARCH process. Technically, the existing properties for the QMLE in the GARCH model need to be reinvestigated to hold uniformly over all possible periods of change. The key results involve a uniform weak Bahadur representation for the estimated parameters, which leads to weak convergence of the test statistic to the supreme of a Gaussian Process. In simulations we show that the test has good size and power for reasonably large time series lengths. We apply the test to Apple asset returns and Bitcoin returns.

==> oldstuff.tex <==
%%%%%%%old
\ignore{
We now show an analogue of (iv) in the proof of Theorem 2.1. in \cite{garch2004}. Let $R := \{(r_1,r_2) \in [0,1]^2: r_1 < r_2, |r_1 - r_2|\ge \kappa\}$. We want to show: For all $\theta\not= \theta^{*}$, there exists a neighbourhood $V(\theta)$ such that
\begin{equation}
    \liminf_{n\to\infty}\inf_{\theta'\in V_k(\theta)}\inf_{(r_1,r_2)\in R}\frac{L_{n,r_1,r_2}^c(\theta')}{r_2-r_1} > L(\theta^{*}).\label{eq:consistencyproof0}
\end{equation}
By Lemma \ref{lemma:truncation}(ii), we have
\[
    \sup_{\theta \in \Theta}\sup_{r\in[0,1]}|L_{n,r}^c(\theta) - L_{n,r}(\theta)| \to 0 \quad a.s.
\]
and thus
\begin{equation}
    \sup_{\theta \in \Theta}\sup_{(r_1,r_2)\in R}|L_{n,r_1,r_2}^c(\theta) - L_{n,r_1,r_2}(\theta)| = O_p(n^{-1}).\label{eq:truncation_likelihood1}
\end{equation}
For $\theta \in \Theta$, $\theta\not= \theta^{*}$ and $k\in\IN$ let $V_k(\theta) := \{\theta' \in \Theta: |\theta'-\theta|_1 < 1/k\}$. Then we have by \reff{eq:truncation_likelihood1}:
\begin{eqnarray}
    && \liminf_{n\to\infty}\inf_{\theta'\in V_k(\theta)}\inf_{(r_1,r_2)\in R}\frac{L_{n,r_1,r_2}^c(\theta')}{r_2-r_1}\nonumber\\
    &\ge& \liminf_{n\to\infty}\inf_{\theta'\in V_k(\theta)}\inf_{(r_1,r_2)\in R}\frac{L_{n,r_1,r_2}(\theta')}{r_2-r_1}\nonumber\\
    &\ge& \liminf_{n\to\infty}\inf_{(r_1,r_2)\in R}\frac{1}{n(r_2-r_1)}\sum_{i=\lfloor nr_1\rfloor+1}^{\lfloor nr_2\rfloor}\inf_{\theta' \in V_k(\theta)}\ell(X_i^2,Y_i,\theta').\label{eq:consistencyproof1}
\end{eqnarray}
Since $W_i := \inf_{\theta'\in V_k(\theta)}\ell(X_i^2,Y_i,\theta)$ is stationary, we have by the ergodic theorem for $\IE W_1 \in \IR \cup \{\infty\}$:
\[
    \liminf_{n\to\infty}\frac{1}{m}\sum_{i=1}^{m}W_i = \IE W_1 \quad a.s.
\]
Since $|r_2 - r_1| \ge \kappa$ implies that $m_n := \lfloor n r_2\rfloor - \lfloor n r_1\rfloor \to \infty$, we conclude that
\[
    \liminf_{n\to\infty}\inf_{(r_1,r_2)\in R}\frac{1}{\lfloor n r_2\rfloor - \lfloor n r_1\rfloor}\sum_{i=1}^{\lfloor n r_2\rfloor - \lfloor n r_1\rfloor}W_i = \IE W_1 \quad a.s.
\]
By stationarity of $W_i$ and since $\sup_{(r_1,r_2)\in R}|\frac{\lfloor n r_2\rfloor - \lfloor n r_1\rfloor}{n(r_2 - r_1)}- 1| \to 0$, we obtain
\begin{equation}
    \liminf_{n\to\infty}\inf_{(r_1,r_2)\in R}\frac{1}{n(r_2 - r_1)}\sum_{i= \lfloor n r_1\rfloor+1}^{\lfloor n r_2\rfloor}W_i = \IE W_1 \quad a.s.\label{eq:consistencyproof2}
\end{equation}
By \reff{eq:consistencyproof1} and \reff{eq:consistencyproof2}, we have
\[
    \liminf_{n\to\infty}\inf_{\theta'\in V_k(\theta)}\inf_{(r_1,r_2)\in R}\frac{L_{n,r_1,r_2}^c(\theta')}{r_2-r_1} \ge \IE \inf_{\theta' \in V_k(\theta)}\ell(X_i^2,Y_i,\theta').
\]
Since $\theta\not= \theta^{*}$ and $\inf_{\theta' \in V_k(\theta)}\ell(X_i^2,Y_i,\theta') \uparrow \ell(X_i^2,Y_i,\theta)$ and \reff{eq:consistencyproofminus1}, the result \reff{eq:consistencyproof0} follows.

The stated consistency now follows from a compactness argument as follows: Let $\varepsilon > 0$ be arbitrary. Define the compact set $\hat \Theta := \Theta \backslash \{\theta \in \Theta: |\theta - \theta^{*}|_1 < \varepsilon\}$. Suppose that $\limsup_{n\to\infty}\sup_{(r_1,r_2)\in R}|\hat \theta_{n,r_1,r_2} - \theta^{*}| \ge 2\varepsilon$. Therefore, there exists a sequence $n_m$ and $(r_1(m),r_2(m)) \in R$ with $\forall m\in\IN: |\hat \theta_{n,r_1,r_2} - \theta^{*}| \ge \varepsilon$.

Since $\hat \Theta$ is compact, there exist $\theta_1,...,\theta_l \in \hat \Theta$ such that $\bigcup_{i=1}^{l}V(\theta_i)$, where $V(\theta_i)$ are the neighbourhoods from \reff{eq:consistencyproof0}. By writing $\inf_{\theta'\in \hat \Theta} = \inf_{i=1,...,l}\inf_{\theta'\in V(\theta_i)}$ and using \reff{eq:consistencyproof0}, we conclude that
\begin{eqnarray}
    &&\liminf_{m\to\infty}L_{n_m,r_1(m),r_2(m)}^c(\hat\theta_{n_m,r_1(m),r_2(m)})\nonumber\\
    &=& \liminf_{m\to\infty}\inf_{\theta' \in \hat \Theta}L_{n_m,r_1(m),r_2(m)}^c(\theta)\nonumber\\
    &\ge& \liminf_{n\to\infty}\inf_{(r_1,r_2)\in R}\inf_{\theta' \in \hat \Theta}\frac{L_{n,r_1,r_2}^c(\theta')}{r_2-r_1} > L(\theta^{*}).\label{eq:consistencyproof3}
\end{eqnarray}
Using the ergodic theorem and \reff{eq:truncation_likelihood1}, we obtain
\begin{equation}
    \lim_{n\to\infty}\sup_{\theta \in \Theta}\sup_{(r_1,r_2)\in R}|\frac{L_{n,r_1,r_2}(\theta^{*})}{r_2-r_1} - L(\theta^{*})| = 0\quad a.s.\label{eq:consistencyproof4}
\end{equation}
Combining \reff{eq:consistencyproof3} and \reff{eq:consistencyproof4} and the minimal property of $\hat \theta_{n,r_1,r_2}$, we obtain
\[
    0 \ge \liminf_{m\to\infty}\big\{L_{n_m,r_1(m),r_2(m)}^c(\hat\theta_{n_m,r_1(m),r_2(m)}) - L_{n_m,r_1(m),r_2(m)}^c(\theta^{*})\big\} > 0,
\]
a contradiction. Thus $\limsup_{n\to\infty}\sup_{(r_1,r_2)\in R}|\hat \theta_{n,r_1,r_2} - \theta^{*}| \le 2\varepsilon$.}
%%%%%%%old

